A Stochastic Game Approach to Masking Fault-Tolerance: Bisimulation and Quantification

We introduce a formal notion of masking fault-tolerance between probabilistic transition systems based on a variant of probabilistic bisimulation (named masking simulation). We also provide the corresponding probabilistic game characterization. Even though these games could be infinite, we propose a symbolic way of representing them, such that it can be decided in polynomial time if there is a masking simulation between two probabilistic transition systems. We use this notion of masking to quantify the level of masking fault-tolerance exhibited by almost-sure failing systems, i.e., those systems that eventually fail with probability 1. The level of masking fault-tolerance of almost-sure failing systems can be calculated by solving a collection of functional equations. We produce this metric in a setting in which the minimizing player behaves in a strong fair way (mimicking the idea of fair environments), and limit our study to memoryless strategies due to the infinite nature of the game. We implemented these ideas in a prototype tool, and performed an experimental evaluation.

==> running_example.tex <==
\section{A Running Example}
	Let us consider a simple example to illustrate our way of modeling and reasoning about faults and fault-tolerance. For the sake of simplicity, in the graphics below, we draw  
Diract distributions using a single arrow, while other distributions are drawn using branched arrows. Fig.~\ref{fig:exam_1_mem_cell} depicts two systems, the leftmost is a simple memory
supporting reading and writing operations,
\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{figs/probMemory2.pdf}
\caption{PTS's for the memory cell} \label{fig:exam_1_mem_cell}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{figs/loopExample.pdf}
\caption{Example of PTS's with loops} \label{fig:exam_2_loop}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{figs/loopExampleGameGraph.pdf}
\caption{Partial Game Graph for the PTS's of Fig.~\ref{fig:exam_2_loop}} \label{fig:loop_game}
\end{figure}

==> symbolic_games.tex <==
\section{Symbolic Games}
	From now on we assume an enumerable set of variables $V = \{v_0, v_1,\dots\}$. The set of Boolean formulas over inequalities (denoted $\mathbb{B}$)
is defined by the following grammar:
\begin{eqnarray}
	\mathbb{B}  & ::= &  \text{true} \mid  \mathbb{B} \wedge \mathbb{B} \mid \neg \mathbb{b} \mid v_i \geq k 
\end{eqnarray}
where $k \in \mathbb{Q}$. 

	Furthermore, given an finite  set $S=\{s_0,\dots,s_{n-1}\}$, we consider a $n$-dimensional vector  $\mathbf{x}_S$  of numeric variables such that $(\mathbf{x}_S)_i = x_i$. We also consider system of equations
of the style $\mathbf{A} \mathbf{x}^T_S = \mathbf{y}$  where: $\mathbf{A}$ is a $n \times n$ matrix such that $\mathbf{A}_{i,j} \in \{0,1\}$ and
$\sum^{n-1}_{j=0}A_{{n-1},j} = 1$. Furthermore, $\mathbf{y}$ is a $n$-dimensional vector satisfying $\sum^{n-1}_{i=0}\mathbf{y}_i = 1$. It is clear that any solution of $\mathbf{A} \mathbf{x}^T_S = \mathbf{y}$
can be identified with a distribution $\mu \in \text{Dist}(S)$, where the value of $x_s$ corresponds to $\mu(s)$
Now, we  introduce the notion of \emph{Symbolic Stochastic  Game}.
\begin{definition} A Symbolic Stochastic Game  is a tuple $G=(V, E, V_{\text{min}}, V_{\text{max}})$ where:
\begin{itemize}
	\item $V$ is a collection of symbolic states, each symbolic state $s$ has a set of free variables, denoted $\text{fv}(s)$,  and each 
	variable $x \in \text{fv}(s)$ has a set of values associate to it, denoted $\text{val}(x)$,
	\item $(V_{\text{max}}, V_{\min})$ is a partition of  $V$,	
	\item $E \subseteq (V \times \mathbb{B} \times V)$ is a collection of edges, each edge $(v, b, v') \in E$ is written $s \xrightarrow{b} s'$,
	\item Each state $v \in V$ may have  associated a system of equations of the type: $\mathbf{A} \mathbf{x}^T_V = \mathbf{y}$ (denoted $\text{Eq}(s)$).
\end{itemize}
\end{definition}
The system of equations associated with states is denoted by $\text{Eq}(s)$, when no system of equations is associated with a state $s$ we just set $\text{Eq}(s) = \bot$. If $\text{Eq}(s) =\bot$
for every $s \in S$, we say that $SG$ is a \emph{Symbolic $2$-Player Game}.

	Intuitively, each symbolic stochastic game represents a stochastic game with more (perhaps infinite) states. 
\begin{definition} A Symbolic Stochastic Game  is a tuple $G=(V, E, V_{\text{min}}, V_{\text{max}})$  we define a stochastic game $G^*=(V^*, E^*, V^*_{\text{min}}, V^*_{\text{max}}, V^*_{R})$
as follows:
\begin{itemize}
	\item $V_{\text{min}}^* = \{v: \text{fv}(v) \rightarrow \text{Val} \mid v \in V_{\text{min}}\}$,
	\item $V_{\text{max}}^* = \{s: \text{fv}(v) \rightarrow \text{Val} \mid v \in V_{\text{max}}\}$,
\end{itemize}
\end{definition}

	


